Video Unsupervised Domain Adaptation with Deep Learning: A Comprehensive Survey

Video analysis tasks such as action recognition have received increasing research interest with growing applications in fields such as smart healthcare, thanks to the introduction of large-scale datasets and deep learning-based representations. However, video models trained on existing datasets suffer from significant performance degradation when deployed directly to real-world applications due to domain shifts between the training public video datasets (source video domains) and real-world videos (target video domains). Further, with the high cost of video annotation, it is more practical to use unlabeled videos for training. To tackle performance degradation and address concerns in high video annotation cost uniformly, the video unsupervised domain adaptation (VUDA) is introduced to adapt video models from the labeled source domain to the unlabeled target domain by alleviating video domain shift, improving the generalizability and portability of video models. This paper surveys recent progress in VUDA with deep learning. We begin with the motivation of VUDA, followed by its definition, and recent progress of methods for both closed-set VUDA and VUDA under different scenarios, and current benchmark datasets for VUDA research. Eventually, future directions are provided to promote further VUDA research. The repository of this survey is provided at https://github.com/xuyu0010/awesome-video-domain-adaptation.

==> abstract_original.tex <==
Video analysis tasks, such as action recognition and video segmentation, have received increasing research interest thanks to their growing application in fields such as autonomous driving and smart healthcare, thanks to the introduction of large-scale datasets and deep learning-based video representations. However, current video models trained on existing datasets suffers from significant performance degradation when deployed directly to real-world applications due to domain shift between the training public video dataset acting as the source video domain and the real-world video data acting as the target video domain. Further, due to the high cost of annotating large-scale real-world video data, it is more practical to obtain unlabeled video data for video model training. To tackle the problem of performance degradation and address concerns in high data annotation cost uniformly, the video unsupervised domain adaptation (VUDA) is introduced which helps video models to be adapted to the unlabeled target video domain from the labeled video source domain by alleviating video domain shift, thus improving the generalizability and portability of video models. This paper surveys the recent progress in VUDA with deep learning. We begin with the motivation of VUDA, followed its definition. We then review methods for both closed-set VUDA and VUDA under different scenarios with different constraints, assumptions and tasks. Further, the benchmark datasets to facilitate current VUDA research are investigated. Eventually, the recent progress of current VUDA works are summarized and insights for future directions of VUDA research are provided to facilitate and promote future VUDA research.
